A Dataset for Tracking Entities in Open Domain Procedural Text

We present the first dataset for tracking state changes in procedural text from arbitrary domains by using an unrestricted (open) vocabulary. For example, in a text describing fog removal using potatoes, a car window may transition between being foggy, sticky,opaque, and clear. Previous formulations of this task provide the text and entities involved,and ask how those entities change for just a small, pre-defined set of attributes (e.g., location), limiting their fidelity. Our solution is a new task formulation where given just a procedural text as input, the task is to generate a set of state change tuples(entity, at-tribute, before-state, after-state)for each step,where the entity, attribute, and state values must be predicted from an open vocabulary. Using crowdsourcing, we create OPENPI1, a high-quality (91.5% coverage as judged by humans and completely vetted), and large-scale dataset comprising 29,928 state changes over 4,050 sentences from 810 procedural real-world paragraphs from WikiHow.com. A current state-of-the-art generation model on this task achieves 16.1% F1 based on BLEU metric, leaving enough room for novel model architectures.

==> sections/custom-commands.tex <==

\newcommand{\ourdata}[1]{\textsc{OpenPI}}


\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0,0.7,0}
\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{0.6,0,0}
\definecolor{Orange}{rgb}{1,0.5,0}
\newcommand{\niket}[1]{\textcolor{Green}{[#1 \textsc{--Niket}]}}
\newcommand{\peter}[1]{\textcolor{Green}{[#1 \textsc{--Peter}]}}
\newcommand{\bhavana}[1]{\textcolor{Green}{[#1 \textsc{--Bhavana}]}}
\newcommand{\dheeraj}[1]{\textcolor{Green}{[#1 \textsc{--Dheeraj}]}}
\newcommand{\keisuke}[1]{\textcolor{Red}{[#1 \textsc{--Keisuke}]}}
\newcommand{\reviewed}[1]{\textcolor{Orange}{[#1]}}


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\newcommand{\vect}[1]{\mathbf{#1}}

\newcommand{\bluebox}[1]{\colorbox{blue!10}{#1}}
\newcommand{\redbox}[1]{\colorbox{red!10}{#1}}
\newcommand{\purplebox}[1]{\colorbox{purple!10}{#1}}
% \newcommand{\bluebox}[1]{{\sethlcolor{blue!10}\hl{#1}}}

% \definecolor{Red}{rgb}{1,0,0}
% \definecolor{Green}{rgb}{0,0.7,0}
% \definecolor{Blue}{rgb}{0,0,1}
% \definecolor{Red}{rgb}{0.6,0,0}
% \definecolor{Orange}{rgb}{1,0.5,0}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newtoggle{draft}
% \toggletrue{draft}
% % \togglefalse{draft}
% \iftoggle{draft}{
% \newcommand{\newresults}[1]{#1}
% \newcommand{\pete}[1]{\textcolor{Blue}{[#1 \textsc{--Pete}]}}
% \newcommand{\niket}[1]{\textcolor{Orange}{[#1 \textsc{--Niket}]}}
% \newcommand{\bhavana}[1]{\textcolor{Green}{[#1 \textsc{--Bhavana}]}}
% \newcommand{\keisuke}[1]{\textcolor{Red}{[#1 \textsc{--Keisuke}]}}
% \newcommand{\todo}[1]{\textcolor{Red}{[\textsc{TODO: }#1 ]}}
% }{
% \newcommand{\peter}[1]{}
% \newcommand{\niket}[1]{}
% \newcommand{\dheeraj}[1]{}
% \newcommand{\todo}[1]{}
% }

\usepackage{amsmath}  % for \mathbb{X} bold X


\def\DG{{\mathcal{G}}}

\newtheorem{theorem}{Definition}[section]

\newcommand{\strikethrough}[1]{\st{#1}}

\newcommand{\namecite}[1]{\citeauthor{#1}~\shortcite{#1}}
\newcommand{\com}[1]{}
\newcommand{\myparagraph}[1]{\vspace{1mm} \noindent {\bf #1: }}
\newcommand{\bfit}[1]{\textbf{\textit{#1}}}
\newcommand{\eat}[1]{}
\mathchardef\mhyphen="2D
\newenvironment{ite}{                     % list without par spacings
     \parskip 0cm \begin{itemize} \parskip 0cm \parsep 0cm \itemsep 0cm \topsep 0cm}{
        \end{itemize}} %  \parskip 0cm}
\newenvironment{enu}{                   % list without par spacings
     \parskip 0cm \begin{list}{}{\parsep 0cm \itemsep 0cm \topsep 0cm}}{
      \end{list}} %  \parskip 0cm}
\newenvironment{des}{                 % list without par spacings
     \parskip 0cm \begin{list}{}{\parsep 0cm \itemsep 0cm \topsep 0cm}}{
      \end{list}} %  \parskip 0cm}
\newenvironment{myenumerate}{                   % list without par spacings
     \parskip 0cm \begin{enumerate}{\parsep 0cm \itemsep 0cm \topsep 0cm}}{
        \end{enumerate}} %  \parskip 0cm}
\newenvironment{myitemize}{                     % list without par spacings
     \parskip 0cm \begin{itemize}{\parsep 0cm \itemsep 0cm \topsep 0cm}}{
        \end{itemize}} %  \parskip 0cm}
\newcommand{\ourdataexpansion}{``What-If Question Answering''}
\newenvironment{myquote}{                   % list without par spacings
  \parskip 0mm \begin{quoting}[vskip=0mm,leftmargin=2mm]}{
\end{quoting}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\olive}[1]{\textcolor{olive}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newenvironment{mycentering}
 {\parskip=0pt\par\nopagebreak\centering}
 {\par\noindent\ignorespacesafterend}


\newcommand{\squishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
\newcommand{\reallysquishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{0.2em} \setlength{\labelwidth}{0.2em}
      \setlength{\labelsep}{0.2em} } }

 \newcommand{\squishend}{
     \end{list} 
 }
 
 
% \newenvironment{myenumerate}
%     {\begin{enumerate}[leftmargin=0.0mm][rightmargin=0.0mm]}
%     {\end{enumerate}
    
% \newenvironment{myitemize}
%     {\begin{itemize}[leftmargin=0.0mm]}
%     {\end{itemize}


\newcommand{\veryshortarrow}[1][4pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\newcommand{\action}[1]{\ul{\textsl{#1}}}

\usepackage{soul}

% \newcommand{\anycond}[1]{\ul{\textsl{#1}}}
\newcommand{\anycond}[1]{\textsl{#1}}

\newcommand{\precond}[1]{\anycond{#1}}
\newcommand{\query}[1]{\textsl{#1}}
\newcommand{\attr}[1]{\emph{#1}}
\newcommand{\entity}[1]{\texttt{#1}}
\newcommand{\postcond}[1]{\anycond{#1}}

\newcommand{\condpair}[2]{\precond{#1} $\veryshortarrow$ \postcond{#2}}


%macros
\newcommand{\xq}{$x_q$\xspace}
\newcommand{\xc}{$x_c$\xspace}
\newcommand{\yipre}{$y_{i}^{\textit{pre}}$\xspace}
\newcommand{\yipost}{$y_{i}^{\textit{post}}$\xspace}
\newcommand{\att}{$\alpha$\xspace}

\definecolor{light-gray}{rgb}{0.95703125,0.953125,0.94921875}%{gray}{0.95}


\newcommand{\frameit}[1]{
\vspace{0.5cm}
\fboxsep10pt
\colorbox{light-gray}
 {
  \begin{minipage}{0.9\textwidth}
    {#1}
  \end{minipage}
 }
\vspace{0.5cm}
}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

==> sections/notes.tex <==
Introduction (pages 0- 1): 
		- motivating example
	Problem statement (1- 1.5):
			- actual problem 
			- simplified problem (with hints in trying to make 1:1)
	Related work (1.5- 2):
		- tracking (open) state changes 
			- (from ProStruct & ProPara)
			- open state changes (visual transformations, can't cite/ overlap w/ acl20)
			- tracking open state changes (what would be most closely related?)
		- generation task
			- 1:N generation problems
			- templated and constrained generation
        - dataset
            - propara, comet, conceptnet, scone, babI
        - table of ticks and crosses for related work
	Dataset (2-3.5):
		- collection and overall statistics (2-2.5)
			- procedure (both modalities)
			- what worked and didn't (modalities, avoiding negations, ...)
			- overall dataset size and statistics
			- sampled data quality
            - url of mturk template
		- quantitative analysis (2.5-3)
        - qualitative analysis (2.5-3)
        - examples (3-3.5)
	Model (3.5-4):
			- T5		
	Evaluation (4-5):
			- Evaluate accuracy automatically and analyze
			- Evaluate consistency automatically and analyze
            - Human evaluation 
			- Successful examples
    Error analysis (5- 5.5):
	Conclusion and future work (5.5-6)
 



Motivation: When tracking open state changes, a fixed set of consistency rules aren't applicable anymore (e.g., foundational SUMO ontology rules on location and existence). Is there a way to automatically measure such consistency errors and can a model learn to track open state changes accurately and consistently.

General errors (these are not inconsistency errors)
- Wrong attribute
- Wrong entity
- Wrong/imagined before state

Inconsistency errors (some types, are there more? -- this is the main focus -- to find examples and discover inconsistency types):
- states after a step `n-1` and before step `n` are not implying something different.
- inconsistency within a step (e..g, opposing attribute values/ antonymous adjectives).

Challenges in tracking open state changes besides inconsistency:

    Entities are open and two entities (bottle) and (shampoo container) can refer to the same.
    Entities are implicit (this was highlighted in Bhavana's document: https://docs.google.com/document/d/14aYbSke2m0JJTh69DO8oYOt0zeqidfckPxaOJRGEs5M/edit)
    Named states (useful for analyzing diversity and redundancy of multiple state changes in an input) are open and can be expressed differently (e.g., location/placement, orientation)
    State changes are open and different entries might imply the same (e.g., example 2 in Bhavana's document) location was in the "jar -> measuring cup" vs. location was in the "measuring cup -> blender" because (a blender might have a jar with measuring cup)
    Context is important (motivation for generation model)





% This necessitates modeling the actions in text and transformations (i.e., state changes) they produce, e.g., when plants absorbs water, then the plants get heavier, more wet, and the water undergoes some movement. Such modeling and reasoning is particularly important with a changing world and an exemplary usecase is procedural text (recipes, how-to guides, etc.) where such a modeling helps in various reasoning end tasks such as automatic execution of biology experiments \cite{mysore2019materials}, cooking recipes \cite{Bollini2012cookingrobot} and everyday activities \cite{Wikihow-sigir2015} \footnote{this is a dummy footnote}.\\




% Text1 traditional-state-change open-state-change
% Text2 traditional-state-change open-state-change
% ...
% \small{

% % GPT2 talktotransformers.com
% % The CRD set up waste trucks Friday on the north side of Enumclaw.
% % https://mosaickg.apps.allenai.org/?l=Cans%20are%20tied%20together%20and%20transported%20to%20a%20recycling%20center.














% We found 78 unique attributes in 20 procedures, another 99 in another set of 20 procedures (of which only 15% overlapped **173-146/ 173**). Some attributes such as state were overloaded. These are implicit examples:
% tied/untied, exposed/protected, room temperature/on fire, whole/cut, unused/in use, liquid/foam, unblended/blended, full/empty, power-on/ power-off
% In an initial experiment with humans, they struggled to do name and put it under state


% Our goal is to relax this restriction and allow an open vocabulary of state changes to be used (referred as \textbf{``Open state changes''}), so that additional aspects of a process can be modeled. 


% end tasks are informed about the entities at different steps in the process. Traditionally, procedural comprehension systems have focused on a small, closed set of state changes. However, real world procedures have a very large space of state changes (estimated at a few hundred well-defined closed attributes, and thousands of attributes without a common name that keep increasing as we move to new domains). This mismatch between state changes limits the modeling potential of existing systems. 

% This is nice.
% Note... While our methods are applicable to any text, we choose procedural text for the experiments because the challenge of modeling and reasoning with a changing world is particularly pertinent in text about processes. 

%To make it possible for users to issue diverse queries over heterogeneous corpora, systems must move away from architectures that require relations to be specified prior to query time in favor of those that aim to discover all possible relations in the text

% Need an example that shows the following phenomena.
% (estimated at a few hundred well-defined closed/explicit attributes e.g. from WordNet, and thousands of attributes without a name/implicit that keep increasing as we move to new domains). This mismatch between state changes ... (note there are other papers that leverage antonym adjectives as attributes).
% implicit
% before: "glassware was spotty.",
% after: "glassware is clear.",
% attribute: "translucency",

% explicit 
% before: "glassware was dry.",	
% after: "glassware is damp.",	
% attribute: "moisture",	(or wetness)

% We found 78 unique attributes in 20 procedures, another 99 in another set of 20 procedures (of which only 15% overlapped **173-146/ 173**). Some attributes such as state were overloaded. These are implicit examples:
% tied/untied, exposed/protected, room temperature/on fire, whole/cut, unused/in use, liquid/foam, unblended/blended, full/empty, power-on/ power-off
% In an initial experiment with humans, they struggled to do name and put it under state







% % Additional paragraph on limitation
% This motivated us to run a pilot study asking turkers to annotate possible state changes in procedural paragraphs from several domains on WikiHow.com (experimental details in \S \ref{sec:experiments}). From this study, we discovered that:

% (i) Real-world text requires a very large number of state changes such as physical attributes (temperature, weight, volume, texture, shape, mass, cleanliness, wetness, etc.) %social attributes (motivated, happy, sad) 
% However, existing systems use a small set of \textit{explicit} state change types (e.g., the state-of-the-art models based on ProPara can only infer create, destroy, and move). 

% (ii) A large set of state changes tend to be \textit{implicit}, e.g., whether something is tied/untied, exposed/protected, on room temperature/on fire, whole/cut liquid/foam, unblended/blended, full/empty etc. It is not possible to meaningfully express these explicitly. However, existing system use a pre-defined ontology of explicit state changes.

% (iii) Different domains (such as health, cooking, etc.), share only about 15\% of the attributes (these tend to be explicit attributes). A majority of the attributes (85\%) are novel (these tend to be implicit attributes). As we strive for more general systems that can model multiple domains, it will be necessary to have an open vocabulary (so that previously unseen implicit changes can also be inferred). However, there are no systems currently that strive towards such an open vocabulary.



% The cans are shredded by a machine and heated.\\
% \textbf{COMET:} BEFORE: Person pickup cans, buy cans, have a machine...\\
% \textbf{COMET:} AFTER: Persons gets burned, person gets dirty...\\

% \noindent Cans are tied together and transported to a recycling center.\\
% \textbf{COMET:} BEFORE: Person needed to be arrested, Person needs to go to recycle center...\\
% \textbf{COMET:} AFTER: Person is arrested, Person gets dirty...\\

% The molten metal is flattened for reuse.\\
% \textbf{COMET:} BEFORE: Person needed to buy a ticket, be in a fight...\\
% \textbf{COMET:} AFTER: Person gets dirty, loses money...\\



% Recently, \cite{wiqa} introduced the \textsc{wiqa} task to predict the effect of \textit{perturbations}.


% How we address that problem.
% This will allow modeling of additional aspects of a process, making downstream applications more informed. This is a challenging problem: (a) there is no large scale dataset that currently supports such inference. (b) context plays a role when dealing with a large number of state changes types e.g., if ``a stone hits a glass'' then the glass would break but this is not the case if ``a soft toy or a sound wave hits the glass''.

